Representative Image Feature Extraction via Contrastive Learning Pretraining for Chest X-ray Report Generation

Medical report generation is a challenging task since it is time-consuming and requires expertise from experienced radiologists. The goal of medical report generation is to accurately capture and describe the image findings. Previous works pretrain their visual encoding neural networks with large datasets in different domains, which cannot learn general visual representation in the specific medical domain. In this work, we propose a medical report generation framework that uses a contrastive learning approach to pretrain the visual encoder and requires no additional meta information. In addition, we adopt lung segmentation as an augmentation method in the contrastive learning framework. This segmentation guides the network to focus on encoding the visual feature within the lung region. Experimental results show that the proposed framework improves the performance and the quality of the generated medical reports both quantitatively and qualitatively.

==> Table/encoder_f1.tex <==
\begin{table}[h]
\centering
\begin{tabular}{crrr}
\hline
\multicolumn{1}{l}{} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} \\ 
\hline
AE                   & 0.451                         & 0.511                      & 0.480                  \\
SimCLR               & 0.480                         & 0.503                      & 0.490                  \\
\hline
\end{tabular}
\caption{Quantitative comparison of different encoder and decoder test on the IU X-Ray dataset. We evaluate the framework performance by matching the Medical Subject Headings (MeSH) tag of the generated and ground truth reports.}
\label{Table:encoder_F1}
\end{table}

==> Table/iu_xray.tex <==

\begin{table}[h]
\centering
\small
\begin{tabular}{cc|rrrrrr}
\hline
\multicolumn{8}{c}{IU X-ray}\\ 
\hline
\multicolumn{2}{c|}{Metrics}                                 & \multicolumn{1}{c}{B-1} & \multicolumn{1}{c}{B-2} & \multicolumn{1}{c}{B-3} & \multicolumn{1}{c}{B-4} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{R-L} \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{LSTM}}        & Scratch  & 0.299                   & 0.185                   & 0.132                   & 0.100                   & 0.134                 & 0.324                   \\
\multicolumn{1}{c|}{}                             & AE       & 0.389                   & 0.233                   & 0.157                   & 0.111                   & 0.154                 & 0.317                   \\
\multicolumn{1}{c|}{}                             & Imagenet & 0.397                   & 0.246                   & 0.170                   & 0.126                   & 0.160                 & \textbf{0.329}          \\
\multicolumn{1}{c|}{}                             & MLC      & 0.410                   & 0.250                   & 0.170                   & 0.123                   & 0.164                 & 0.325                   \\
\cline{2-8}
\multicolumn{1}{c|}{}                             & SimCLR   & \textbf{0.426}          & \textbf{0.265}          & \textbf{0.181}          & \textbf{0.131}          & 0.168                 & 0.326                   \\
\multicolumn{1}{c|}{}                             & MoCo     & 0.425                   & 0.260                   & 0.177                   & 0.128                   & \textbf{0.169}        & 0.326                   \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{GRU}}         & Scratch  & 0.351                   & 0.221                   & 0.156                   & 0.117                   & 0.153                 & 0.333                   \\
\multicolumn{1}{c|}{}                             & AE       & 0.389                   & 0.241                   & 0.166                   & 0.121                   & 0.161                 & 0.332                   \\
\multicolumn{1}{c|}{}                             & Imagenet & 0.417                   & 0.254                   & 0.173                   & 0.124                   & 0.165                 & 0.328                   \\
\multicolumn{1}{c|}{}                             & MLC      & 0.412                   & \textbf{0.263}          & \textbf{0.189}          & \textbf{0.145}          & \textbf{0.169}        & \textbf{0.341}          \\
\cline{2-8}
\multicolumn{1}{c|}{}                             & SimCLR   & 0.423                   & 0.259                   & 0.175                   & 0.126                   & 0.166                 & 0.327                   \\
\multicolumn{1}{c|}{}                             & MoCo     & \textbf{0.424}          & 0.259                   & 0.174                   & 0.124                   & \textbf{0.169}        & 0.331                   \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{Transformer}} & Scratch  & 0.404                   & 0.249                   & 0.172                   & 0.126                   & 0.161                 & 0.320                   \\
\multicolumn{1}{c|}{}                             & AE       & 0.417                   & 0.273                   & 0.195                   & 0.148                   & \textbf{0.176}        & 0.361                   \\
\multicolumn{1}{c|}{}                             & Imagenet & 0.420                   & 0.256                   & 0.175                   & 0.127                   & 0.167                 & 0.326                   \\
\multicolumn{1}{c|}{}                             & MLC      & 0.423                   & 0.270                   & 0.190                   & 0.141                   & \textbf{0.176}        & 0.359                   \\
\cline{2-8}
\multicolumn{1}{c|}{}                             & SimCLR   & \textbf{0.456}          & \textbf{0.289}          & \textbf{0.202}          & \textbf{0.150}          & \textbf{0.176}        & \textbf{0.362}          \\
\multicolumn{1}{c|}{}                             & MoCo     & 0.426                   & 0.259                   & 0.175                   & 0.126                   & 0.168                 & 0.325                   \\
\hline
\end{tabular}
\caption{Quantitative comparison of different encoder and decoder test on the IU X-Ray dataset. B-n, M, and R-L are short for BLEU-n, METEOR, and ROUGE-L, respectively.}
\label{Table:iu-xray}
\end{table}


==> Table/mimic_cxr.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{cc|rrrrrr}
\hline
\multicolumn{8}{c}{MIMIC-CXR}\\ 
\hline
\multicolumn{2}{c|}{Metrics}                                 & \multicolumn{1}{c}{B-1} & \multicolumn{1}{c}{B-2} & \multicolumn{1}{c}{B-3} & \multicolumn{1}{c}{B-4} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{R-L} \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{LSTM}}        & Scratch  & 0.312                   & 0.193                   & 0.130                   & 0.092                   & 0.128                 & 0.272                   \\
\multicolumn{1}{c|}{}                             & AE       & 0.282                   & 0.174                   & 0.117                   & 0.083                   & 0.119                 & 0.264                   \\
\multicolumn{1}{c|}{}                             & Imagenet & 0.309                   & 0.193                   & 0.131                   & 0.094                   & 0.130                 & 0.276                   \\
\cline{2-8}
\multicolumn{1}{c|}{}                             & SimCLR   & \textbf{0.330}          & \textbf{0.206}          & \textbf{0.139}          & \textbf{0.099}          & \textbf{0.134}        & \textbf{0.278}          \\
\multicolumn{1}{c|}{}                             & MoCo     & 0.309                   & 0.191                   & 0.128                   & 0.091                   & 0.127                 & 0.270                   \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{GRU}}         & Scratch  & 0.309                   & 0.193                   & 0.130                   & 0.093                   & 0.128                 & 0.274                   \\
\multicolumn{1}{c|}{}                             & AE       & 0.299                   & 0.184                   & 0.124                   & 0.088                   & 0.123                 & 0.270                   \\
\multicolumn{1}{c|}{}                             & Imagenet & 0.313                   & 0.196                   & 0.132                   & 0.095                   & 0.129                 & 0.275                   \\
\cline{2-8}
\multicolumn{1}{c|}{}                             & SimCLR   & \textbf{0.327}          & \textbf{0.204}          & \textbf{0.137}          & \textbf{0.098}          & \textbf{0.134}        & \textbf{0.278}          \\
\multicolumn{1}{c|}{}                             & MoCo     & 0.309                   & 0.190                   & 0.127                   & 0.090                   & 0.126                 & 0.269                   \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{Transformer}} & Scratch  & 0.211                   & 0.132                   & 0.090                   & 0.064                   & 0.105                 & 0.250                   \\
\multicolumn{1}{c|}{}                             & AE       & 0.316                   & 0.186                   & 0.119                   & 0.081                   & 0.119                 & 0.243                   \\
\multicolumn{1}{c|}{}                             & Imagenet & 0.270                   & 0.166                   & 0.109                   & 0.076                   & 0.114                 & 0.255                   \\
\cline{2-8}
\multicolumn{1}{c|}{}                             & SimCLR   & \textbf{0.343}          & \textbf{0.208}          & \textbf{0.137}          & \textbf{0.095}          & \textbf{0.132}        & 0.260                   \\
\multicolumn{1}{c|}{}                             & MoCo     & 0.334                   & 0.203                   & 0.133                   & 0.091                   & 0.129                 & \textbf{0.261}          \\
\hline
\end{tabular}
\caption{Quantitative comparison of different encoder and decoder test on the MIMIC-CXR dataset. B-n, M, and R-L are short for BLEU-n, METEOR, and ROUGE-L, respectively.}
\label{Table:mimic-cxr}
\end{table}


==> Table/mix.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\small
\begin{tabular}{cc|rrrrrr|rrrrrr}
\multicolumn{2}{c|}{Dataset}                                 & \multicolumn{6}{c|}{IU X-ray}                                                                                                                            & \multicolumn{6}{c}{MIMIC-CXR}                                                                                                                           \\ \hline
\multicolumn{2}{c|}{Metrics}                                 & \multicolumn{1}{c}{B-1} & \multicolumn{1}{c}{B-2} & \multicolumn{1}{c}{B-3} & \multicolumn{1}{c}{B-4} & \multicolumn{1}{c}{M} & \multicolumn{1}{c|}{R-L} & \multicolumn{1}{c}{B-1} & \multicolumn{1}{c}{B-2} & \multicolumn{1}{c}{B-3} & \multicolumn{1}{c}{B-4} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{R-L} \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{LSTM}}        & Scratch  & 0.299                   & 0.185                   & 0.132                   & 0.100                   & 0.134                 & 0.324                    & 0.312                   & 0.193                   & 0.130                   & 0.092                   & 0.128                 & 0.272                   \\
\multicolumn{1}{c|}{}                             & AE       & 0.389                   & 0.233                   & 0.157                   & 0.111                   & 0.154                 & 0.317                    & 0.282                   & 0.174                   & 0.117                   & 0.083                   & 0.119                 & 0.264                   \\
\multicolumn{1}{c|}{}                             & Imagenet & 0.419                   & 0.265                   & 0.188                   & 0.142                   & 0.169                 & 0.351                    & 0.309                   & 0.193                   & 0.131                   & 0.094                   & 0.130                 & 0.276                   \\
\multicolumn{1}{c|}{}                             & MLC      & 0.310                   & 0.192                   & 0.138                   & 0.106                   & 0.138                 & 0.321                    & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}   \\
\multicolumn{1}{c|}{}                             & SimCLR   & 0.426                   & 0.265                   & 0.181                   & 0.131                   & 0.168                 & 0.326                    & 0.330                   & 0.206                   & 0.139                   & 0.099                   & 0.134                 & 0.278                   \\
\multicolumn{1}{c|}{}                             & MoCo     & 0.425                   & 0.260                   & 0.177                   & 0.128                   & 0.169                 & 0.326                    & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}   \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{GRU}}         & Scratch  & 0.421                   & 0.258                   & 0.176                   & 0.127                   & 0.166                 & 0.330                    & 0.309                   & 0.193                   & 0.130                   & 0.093                   & 0.128                 & 0.274                   \\
\multicolumn{1}{c|}{}                             & AE       & 0.389                   & 0.241                   & 0.166                   & 0.121                   & 0.161                 & 0.332                    & 0.299                   & 0.184                   & 0.124                   & 0.088                   & 0.123                 & 0.270                   \\
\multicolumn{1}{c|}{}                             & Imagenet & 0.417                   & 0.254                   & 0.173                   & 0.124                   & 0.165                 & 0.328                    & 0.313                   & 0.196                   & 0.132                   & 0.095                   & 0.129                 & 0.275                   \\
\multicolumn{1}{c|}{}                             & MLC      & 0.412                   & 0.263                   & 0.189                   & 0.145                   & 0.169                 & 0.341                    & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}   \\
\multicolumn{1}{c|}{}                             & SimCLR   & 0.423                   & 0.259                   & 0.175                   & 0.126                   & 0.166                 & 0.327                    & 0.327                   & 0.204                   & 0.137                   & 0.098                   & 0.134                 & 0.278                   \\
\multicolumn{1}{c|}{}                             & MoCo     & 0.424                   & 0.259                   & 0.174                   & 0.124                   & 0.169                 & 0.331                    & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}   \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{Transformer}} & Scratch  & 0.404                   & 0.249                   & 0.172                   & 0.126                   & 0.161                 & 0.320                    & 0.211                   & 0.132                   & 0.090                   & 0.064                   & 0.105                 & 0.250                   \\
\multicolumn{1}{c|}{}                             & AE       & 0.417                   & 0.273                   & 0.195                   & 0.148                   & 0.176                 & 0.361                    & 0.316                   & 0.186                   & 0.119                   & 0.081                   & 0.119                 & 0.243                   \\
\multicolumn{1}{c|}{}                             & Imagenet & 0.420                   & 0.256                   & 0.175                   & 0.127                   & 0.167                 & 0.326                    & 0.270                   & 0.166                   & 0.109                   & 0.076                   & 0.114                 & 0.255                   \\
\multicolumn{1}{c|}{}                             & MLC      & 0.423                   & 0.270                   & 0.190                   & 0.141                   & 0.176                 & 0.359                    & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}   \\
\multicolumn{1}{c|}{}                             & SimCLR   & 0.456                   & 0.289                   & 0.202                   & 0.150                   & 0.176                 & 0.362                    & 0.343                   & 0.208                   & 0.137                   & 0.095                   & 0.132                 & 0.260                   \\
\multicolumn{1}{c|}{}                             & MoCo     & 0.405                   & 0.243                   & 0.162                   & 0.115                   & 0.166                 & 0.314                    & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}  
\end{tabular}
\end{table}

==> Table/seg_exp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\small
\begin{tabular}{c|cl|rrrrrr}
\hline
Dataset                    & \multicolumn{2}{c|}{Method}                                & \multicolumn{1}{c}{B-1} & \multicolumn{1}{c}{B-2} & \multicolumn{1}{c}{B-3} & \multicolumn{1}{c}{B-4} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{R-L} \\ \hline
\multirow{6}{*}{IU X-ray}  & \multicolumn{1}{c|}{\multirow{2}{*}{LSTM}}        & SimCLR & 0.426                   & 0.265                   & 0.181                   & 0.131                   & 0.168                 & 0.326                   \\
                           & \multicolumn{1}{c|}{}                             & w/ LM  & 0.431                   & 0.268                   & 0.185                   & 0.137                   & 0.172                 & 0.332                   \\ \cline{2-9} 
                           & \multicolumn{1}{c|}{\multirow{2}{*}{GRU}}         & SimCLR & 0.423                   & 0.259                   & 0.175                   & 0.126                   & 0.166                 & 0.327                   \\
                           & \multicolumn{1}{c|}{}                             & w/ LM  & 0.415                   & 0.255                   & 0.174                   & 0.127                   & 0.165                 & 0.331                   \\ \cline{2-9} 
                           & \multicolumn{1}{c|}{\multirow{2}{*}{Transformer}} & SimCLR & 0.456                   & 0.289                   & 0.202                   & 0.150                   & 0.176                 & 0.362                   \\
                           & \multicolumn{1}{c|}{}                             & w/ LM  & 0.448                   & 0.282                   & 0.195                   & 0.141                   & 0.176                 & 0.340                   \\ \hline
\multirow{6}{*}{MIMIC-CXR} & \multicolumn{1}{c|}{\multirow{2}{*}{LSTM}}        & SimCLR & 0.330                   & 0.206                   & 0.139                   & 0.099                   & 0.134                 & 0.278                   \\
                           & \multicolumn{1}{c|}{}                             & w/ LM  & 0.325                   & 0.203                   & 0.138                   & 0.098                   & 0.134                 & 0.278                   \\ \cline{2-9} 
                           & \multicolumn{1}{c|}{\multirow{2}{*}{GRU}}         & SimCLR & 0.327                   & 0.204                   & 0.137                   & 0.098                   & 0.134                 & 0.278                   \\
                           & \multicolumn{1}{c|}{}                             & w/ LM  & 0.335                   & 0.209                   & 0.140                   & 0.100                   & 0.136                 & 0.279                   \\ \cline{2-9} 
                           & \multicolumn{1}{c|}{\multirow{2}{*}{Transformer}} & SimCLR & 0.343                   & 0.208                   & 0.137                   & 0.095                   & 0.132                 & 0.260                   \\
                           & \multicolumn{1}{c|}{}                             & w/ LM  & 0.325                   & 0.198                   & 0.130                   & 0.090                   & 0.129                 & 0.265
                                             \\ \hline
\end{tabular}
\caption{Quantitative comparison for encoder with and without adding Lung Masking (LM) over IU X-Ray dataset and MIMIC-CXR dataset. B-n, M, and R-L are short for BLEU-n, METEOR, and ROUGE-L, respectively. Higher value is better in all columns.}
\label{Table:seg_exp}
\end{table}

==> hacks/many-authors-hack.tex <==
%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}
